An Inexact Proximal Path-Following Algorithm for Constrained Convex Minimization

Many scientific and engineering applications feature nonsmooth convex minimization problems over convex sets. In this paper, we address an important instance of this broad class where we assume that the nonsmooth objective is equipped with a tractable proximity operator and that the convex constraint set affords a self-concordant barrier. We provide a new joint treatment of proximal and self-concordant barrier concepts and illustrate that such problems can be efficiently solved, without the need of lifting the problem dimensions, as in disciplined convex optimization approach. We propose an inexact path-following algorithmic framework and theoretically characterize the worst-case analytical complexity of this framework when the proximal subproblems are solved inexactly. To show the merits of our framework, we apply its instances to both synthetic and real-world applications, where it shows advantages over standard interior point methods. As a by-product, we describe how our framework can obtain points on the Pareto frontier of regularized problems with self-concordant objectives in a tuning free fashion.

==> siopt2013_PFPNT_bib.tex <==
\begin{thebibliography}{10}

\bibitem{Banerjee2008}
{\sc Banerjee, O., El~Ghaoui, L., and d'Aspremont, A.}
\newblock Model selection through sparse maximum likelihood estimation for
  multivariate gaussian or binary data.
\newblock {\em Journal of Machine Learning Research}, 9, (2008), 485--516.

\bibitem{Bank1983}
{\sc Bank, B., Guddat, J., Klatte, D., Kummer, B., and Tammer, K.}
\newblock {\em {N}on-{L}inear {P}arametric {O}ptimization}.
\newblock Birkhauser Verlag, 1983.

\bibitem{Bansal2004}
{\sc Bansal, N., Blum, A., and Chawla, S.}
\newblock {C}orrelation {C}lustering.
\newblock {\em Machine Learning}, 56, (2004), 89--113.

\bibitem{Bauschke2011}
{\sc Bauschke, H., and Combettes, P.}
\newblock {\em Convex analysis and monotone operators theory in {H}ilbert
  spaces}.
\newblock Springer-Verlag, 2011.

\bibitem{Beck2009}
{\sc Beck, A., and Teboulle, M.}
\newblock {A} {F}ast {I}terative {S}hrinkage-{T}hresholding {A}lgorithm for
  {L}inear {I}nverse {P}roblems.
\newblock {\em SIAM J. Imaging Sciences}, 2(1), (2009), 183--202.

%\bibitem{Becker2011}
%{\sc Becker, S., Bobin, J., and Cand\`{e}s, E.}
%\newblock {NESTA}: a fast and accurate first-order method for sparse recovery.
%\newblock {\em SIAM J. Imaging Science}, 4(1), (2011), 1--39.

\bibitem{Becker2011b}
{\sc Becker, S., Cand\`{e}s, E., and Grant, M.}
\newblock Templates for convex cone problems with applications to sparse signal
  recovery.
\newblock {\em Mathematical Programming Computation}, 3, (2011), 165--218.

\bibitem{BenTal2004}
{\sc Ben-Tal, A., and Nemirovski, A.}
\newblock {\em Lectures on Modern Convex Optimization: Analysis, Algorithms,
  and Engineering Applications}.
\newblock SIAM, 2001.

\bibitem{VanDenBerg2008}
{\sc Berg, E. V.~D., and Friedlander, M.~P.}
\newblock Probing the {Pareto} frontier for basic pursuit solutions.
\newblock {\em SIAM J. Sci. Comput.}, 31(2), (2008), 890--912.

\bibitem{bhaskar2012atomic}
{\sc Bhaskar, B.~N., Tang, G., and Recht, B.}
\newblock Atomic norm denoising with applications to line spectral estimation.
\newblock {\em arXiv preprint arXiv:1204.0562}, (2012).

\bibitem{Boyd1994}
{\sc Boyd, S., Ghaoui, L., Feron, E., and Balakrishnan, V.}
\newblock {\em Linear matrix inequalities in system and control theory},
  vol.~14.
\newblock SIAM, 1994.

\bibitem{Dempster1972}
{\sc Dempster, A.~P.}
\newblock Covariance selection.
\newblock {\em Biometrics}, 28, (1972), 157--175.

\bibitem{Facchinei2003}
{\sc Facchinei, F., and Pang, J.-S.}
\newblock {\em Finite-dimensional variational inequalities and complementarity
  problems}, vol.~1-2.
\newblock Springer-Verlag, 2003.

\bibitem{Fiacco1983}
{\sc Fiacco, A.}
\newblock {\em {I}ntroduction to sensitivity and stability analysis in
  nonlinear programming}.
\newblock Academic Press, New York, 1983.

\bibitem{Grant2006}
{\sc Grant, M., Boyd, S., and Ye, Y.}
\newblock Disciplined convex programming.
\newblock In {\em Global Optimization: From Theory to Implementation},
  L.~Liberti and N.~Maculan, Eds., Nonconvex Optimization and its Applications.
  Springer, (2006), 155--210.

\bibitem{Guddat1990}
{\sc Guddat, J., Vasquez, F.~G., and Jongen, H.}
\newblock {\em {P}arametric {O}ptimization: {S}ingularities, {P}athfollowing
  and {J}umps}.
\newblock Teubner, Stuttgart, 1990.

\bibitem{Hale2008}
{\sc Hale, E., Yin, W., and Zhang, Y.}
\newblock Fixed-point continuation for $\ell_1$-minimization: methodology and
  convergence.
\newblock {\em SIAM J. Optim.}, 19(3), (2008), 1107--1130.

\bibitem{Harmany2012}
{\sc Harmany, Z., Marcia, R., and Willett, R.~M.}
\newblock This is {SPIRAL-TAP}: Sparse poisson intensity reconstruction algorithms - theory and practice.
\newblock {\em IEEE Transactions on Image Processing (under review)}, (2012),   1--13.

\bibitem{Hassibi1999}
{\sc Hassibi, A., How, J., and Boyd, S.}
\newblock A path following method for solving bmi problems in control.
\newblock In {\em Proceedings of American Control Conference}, 2, (1999), 1385--1389.

\bibitem{Jalali2012}
{\sc Jalali, A., and Srebro, N.}
\newblock Clustering using max-norm constrained optimization.
\newblock In {\em Proc. of International Conference on Machine Learning
  (ICML2012)}, (2012), 1--17.

\bibitem{Kyrillidis2013}
{\sc Kyrillidis, A., and Cevher, V.}
\newblock Fast proximal algorithms for self-concordant function minimization
  with application to sparse graph selection.
\newblock {\em Proc. of the 38th International Conference on Acoustics, Speech,
  and Signal Processing (ICASSP)}, (2013), 1--5.

\bibitem{Lu2010}
{\sc Lu, Z.}
\newblock Adaptive first-order methods for general sparse inverse covariance
  selection.
\newblock {\em SIAM J. Matrix Anal. \& Appl.} 31(4), (2010), 2000--2016.

%\bibitem{Nemirovski2009}
%{\sc Nemirovski, A., and Todd, M.}
%\newblock Interior-point methods for optimization.
%\newblock {\em Acta Numerica},  xx\/} (2009), 1--44.

\bibitem{Nemirovski2009}
{\sc Nemirovski, A.~S., and Todd, M.~J.}
\newblock Interior-point methods for optimization.
\newblock {\em Acta Numerica}, 17(1), (2008), 191--234.

\bibitem{Nesterov2004}
{\sc Nesterov, Y.}
\newblock {\em {I}ntroductory lectures on convex optimization: a basic course},
  vol.~87 of {\em Applied Optimization}.
\newblock Kluwer Academic Publishers, 2004.

\bibitem{Nesterov2007}
{\sc Nesterov, Y.}
\newblock Gradient methods for minimizing composite objective function.
\newblock {\em CORE Discussion paper}, 76, (2007).

\bibitem{Nesterov1994}
{\sc Nesterov, Y., and Nemirovski, A.}
\newblock {\em Interior-point Polynomial Algorithms in Convex Programming}.
\newblock Society for Industrial Mathematics, 1994.

\bibitem{nesterov1997self}
{\sc Nesterov, Y.~E., and Todd, M.~J.}
\newblock Self-scaled barriers and interior-point methods for convex
  programming.
\newblock {\em Mathematics of Operations Research}, 22(1), (1997), 1--42.

\bibitem{Nocedal2006}
{\sc Nocedal, J., and Wright, S.}
\newblock {\em {N}umerical {O}ptimization}, 2~ed.
\newblock Springer Series in Operations Research and Financial Engineering.
  Springer, 2006.

\bibitem{Ravikumar2011}
{\sc Ravikumar, P., Wainwright, M.~J., Raskutti, G., and Yu, B.}
\newblock High-dimensional covariance estimation by minimizing $\ell_1$-penalized
  log-determinant divergence.
\newblock {\em Electron. J. Statist.}, 5, (2011), 935--988.

\bibitem{Rockafellar1970}
{\sc Rockafellar, R.~T.}
\newblock {\em {C}onvex {A}nalysis}, vol.~28 of {\em Princeton Mathematics
  Series}.
\newblock Princeton University Press, 1970.

\bibitem{Roos2006}
{\sc Roos, C., Terlaky, T., and Vial, J.-P.}
\newblock {\em Interior Point Methods for Linear Optimization}.
\newblock Springer Science, Heidelberg/Boston, 2006.
\newblock (Note: This book is a significantly revised new edition of Interior
  Point Approach to Linear Optimization: Theory and Algorithms).

\bibitem{Scheinberg2009}
{\sc Scheinberg, K., and Rish, I.}
\newblock {SINCO}- a greedy coordinate ascent method for sparse inverse covariance
  selection problem.
\newblock {\em Optimization-online (\url{http://www.optimization-online.org/DB_FILE/2009/07/2359.pdf})}, (2009).

\bibitem{Stadler2012}
{\sc St\"{a}dler, N., B\"{u}lmann, P., and de~Geer, S.~V.}
\newblock $l_1$-penalization for mixture regression models.
\newblock {\em Tech. Report.}, (2012), 1--35.

\bibitem{Sturm1999}
{\sc Sturm, F.}
\newblock Using {SeDuMi} 1.02: A {M}atlab toolbox for optimization over symmetric
  cones.
\newblock {\em Optim. Methods Software}, 11-12, (1999), 625--653.

\bibitem{tang2012compressed}
{\sc Tang, G., Bhaskar, B.~N., Shah, P., and Recht, B.}
\newblock Compressed sensing off the grid.
\newblock {\em arXiv preprint arXiv:1207.6053}, (2012).

\bibitem{TranDinh2012c}
{\sc Tran-Dinh, Q., Necoara, I., Savorgnan, C., and Diehl, M.}
\newblock {A}n {I}nexact {P}erturbed {P}ath-{F}ollowing {M}ethod for
  {L}agrangian {D}ecomposition in {L}arge-{S}cale {S}eparable {C}onvex
  {O}ptimization.
\newblock {\em SIAM J. Optim.}, 23(1), (2013), 95--125.

\bibitem{TranDinh2013c}
{\sc Tran-Dinh, Q., Kyrillidis, A., and Cevher, V.}
\newblock Composite self-concordant minimization.
\newblock Tech. report, Lab. for Information and Inference Systems (LIONS),
  EPFL, Switzerland, CH-1015 Lausanne, Switzerland, (2013), 1--42.

\bibitem{TranDinh2013a}
{\sc Tran-Dinh, Q., Kyrillidis, A., and Cevher, V.}
\newblock A proximal newton framework for composite minimization: {G}raph
  learning without {C}holesky decompositions and matrix inversions.
\newblock {\em JMLR W\& CP}, 28(2), (2013), 271--279.

\bibitem{Tutunku2003}
{\sc T\"{u}t\"{u}nk\"{u}, R., Toh, K., and Todd, M.}
\newblock Solving semidefinite-quadratic-linear programs using {SDPT3}.
\newblock {\em Math. Program.}, 95, (2003), 189--217.

\bibitem{Wright1997}
{\sc Wright, S.}
\newblock {\em {P}rimal-{D}ual {I}nterior-{P}oint {M}ethods}.
\newblock {SIAM} Publications, Philadelphia, 1997.

\end{thebibliography}

